PeleLM-FDF Large Eddy Simulator of Turbulent Combustion

A new computational methodology, termed "PeleLM-FDF" is developed and utilized for high fidelity large eddy simulation (LES) of complex turbulent combustion systems. This methodology is constructed via a hybrid scheme combining the Eulerian PeleLM base flow solver with the Lagrangian Monte Carlo simulator of the filtered density function (FDF) for the subgrid scale reactive scalars. The resulting methodology is capable of simulating some of the most intricate physics of complex turbulence-combustion interactions. This is demonstrated by LES of a non-premixed CO/H$_2$ temporally evolving jet flame. The chemistry is modelled via a skeletal kinetics model, and the results are appraised via detail a posteriori comparisons against direct numerical simulation (DNS) data of the same flame. Excellent agreements are observed for the time evolution of various statistics of the thermo-chemical quantities, including the manifolds of the multi-scalar mixing. The new methodology is capable of capturing the complex phenomena of flame-extinction and re-ignition at a 1/512 of the computational cost of the DNS. The high fidelity and the computational affordability of the new PeleLM-FDF solver warrants its consideration for LES of practical turbulent combustion systems.

==> deleted.tex <==


Keep this for Thesis:

The particle number density decreases significantly in regions of low density such as reaction zone, \cite{Pope85} so it is an open question how to deal with particle filtering with AMR in a low-density regions.  One possible choice is to increase $\Delta_E$ so that there are sufficient particles to construct statistics.  However, by doing so, the dissipative error increases leading to less accurate evaluation of the filtered quantities.  Another possibility is to generate new particles in the low particle density regions. This choice might be quite involved since newly generated particles should not affect the overall statistics. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The comparison of velocity statistics with measured data are shown in Figs. \ref{fig:RU}-\ref{fig:RW}, and show favorable agreement. 
\begin{figure}
    \centering
    \includegraphics[width=0.2\textwidth]{Figures/bar_u_05000.eps}
    \includegraphics[width=0.2\textwidth]{Figures/bar_u_10000.eps}
    \includegraphics[width=0.2\textwidth]{Figures/bar_u_15000.eps}
    \includegraphics[width=0.2\textwidth]{Figures/bar_u_20000.eps}
    \caption{Reynolds-averaged and RMS values of velocity component $u$ ($\circ$: mean DNS, $-$: mean LES-FDF, $\square$: total RMS in DNS, $\textrm{-} \, \textrm{-}$: resolved RMS in LES-FDF)}
    \label{fig:RU}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.2\textwidth]{Figures/bar_v_05000.eps}
    \includegraphics[width=0.2\textwidth]{Figures/bar_v_10000.eps}
    \includegraphics[width=0.2\textwidth]{Figures/bar_v_15000.eps}
    \includegraphics[width=0.2\textwidth]{Figures/bar_v_20000.eps}
    \caption{Reynolds-averaged and RMS values of velocity component $v$ ($\circ$: mean DNS, $-$: mean LES-FDF, $\square$: total RMS in DNS, $\textrm{-} \, \textrm{-}$: resolved RMS in LES-FDF)}
    \label{fig:RV}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.2\textwidth]{Figures/bar_w_05000.eps}
    \includegraphics[width=0.2\textwidth]{Figures/bar_w_10000.eps}
    \includegraphics[width=0.2\textwidth]{Figures/bar_w_15000.eps}
    \includegraphics[width=0.2\textwidth]{Figures/bar_w_20000.eps}
    \caption{Reynolds-averaged and RMS values of velocity component $w$ ($\circ$: mean DNS, $-$: mean LES-FDF, $\square$: total RMS in DNS, $\textrm{-} \, \textrm{-}$: resolved RMS in LES-FDF)}
    \label{fig:RW}
\end{figure}

\be
\label{EQ:SGSStress}
\Sigma_{ij} - \frac{1}{3}\Sigma_{mm}\delta_{ij} = \mu_t \lp \frac{\prt \la u_{i}\ra_{L}}{\prt x_j}+\frac{\prt \la u_{j}\ra_{L}}{\prt
x_i}-\frac{2}{3}\frac{\prt \la u_{m}\ra_{L}}{\prt x_m}\,\delta_{ij}\rp, \ \ \
J^{k}_j = -\gamma_t \frac{\prt \la \phi_{k} \ra_{L}}{\prt x_j},
\ee

where $\gamma_t = \mu_t / \sigma$ is the turbulent diffusion coefficient in which $\sigma$ is the subgrid Schmidt/Prandtl number, {\color{red} Arash: what's the value of $\sigma$? how did you calculate it? Aidyn: $\sigma = 0.7$ is constant} and turbulent viscosity coefficient $\mu_t$. The latter one is calculated using the Vreman's model~\cite{Vreman2004Eddy}.

To fully utilize Monte Carlo for FDF we have modified the original algorithm. In the new algorithm \ref{alg:PeleLM-FDF}, $A$ is an advection operator and $D$ is a diffusion operator. Note that in the PeleLM-FDF algorithm \ref{alg:PeleLM-FDF}, steps \ref{line2}-\ref{line3} are the Lagrangian Monte Carlo. Step \ref{line4} is a prediction of a scalar variables, that involves implicit diffusion advancement, while scalars at step \ref{line5} undergo a fully explicit update, so nether linear nor non-linear equations solver is not required.W The reason for this convenient update is that the diffusion operator is constructed using scalars predicted in step \ref{line4}, while source term is constructed from particle data in step \ref{line3} as $\la \rho S_k \ra^{n+\frac{1}{2}}_{\ell, MC} = \dfrac{1}{2} \lp \la \rho S_k \ra^{n+1}_{\ell, MC} + \la \rho S_k \ra^{n}_{\ell, MC} \rp$. By doing so, we can not fully exploit SDC method \cite{Nonaka2012Deferred, Hamon2019Concurrent} for scalar equations, and the time integration of scalars becomes conditionally stable due to explicit chemical source term treatment.  Nevertheless, the accuracy of the algorithm is second order in time, which is a typical for the most low Mach simulations. 

\begin{algorithm}
\caption{PeleLM-FDF algorithm}
\label{alg:PeleLM-FDF}
\begin{algorithmic}[1]
\STATE\label{line1}{Calculate the velocity filed via PeleLM.}
\STATE\label{line2}{Advance MC procedure by solving equations (\ref{EQ:MC1}) and (\ref{EQ:MC2})}
\STATE\label{line3}{Construct ensemble averaged scalars $\la \bphi \ra_{L, MC}$, density $\la \rho \ra_{\ell, MC}$ and source terms $\la \bf{S} \ra_{L, MC}$ from particle data $\bphi^{+}$ at new time layer using (\ref{EQ:Ensavg}) and (\ref{EQ:EnsavgRHO})}
\STATE\label{line4}{Advance advection and diffusion of scalars \\
$\dfrac{ \la \rho \ra_{\ell}^{n+1} \la \phi_{k}\ra_{L}^{n+1, *} - \la \rho \ra_{\ell}^{n} \la \phi_{k}\ra_{L}^{n}}{ \Delta t} = A^{n} + \dfrac{1}{2} \lp D^{n} + D^{n+1, *} \rp $ }
\STATE\label{line5}{Advance chemical reaction of scalars \\
$\dfrac{ \la \rho \ra_{\ell}^{n+1} \la \phi_{k}\ra_{L}^{n+1} - \la \rho \ra_{\ell}^{n} \la \phi_{k}\ra_{L}^{n}}{ \Delta t} = A^{n} + \dfrac{1}{2} \lp D^{n} + D^{n+1, *} \rp  + \la \rho S_k \ra^{n+\frac{1}{2}}_{\ell, MC}$}
\STATE\label{line6}{Advance velocities and pressure}
\end{algorithmic}
\end{algorithm}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\textwidth]{Figures/JointPDF.png}
    \caption{Joint probability density function of mixture fraction and $Y_{CO_2}$ in plane $y=0$ }
    \label{fig:JPDF}
\end{figure}



\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=0.24\textwidth]{Figures/bar_Z_05000.eps}
    \includegraphics[width=0.24\textwidth]{Figures/bar_Z_10000.eps}
    \includegraphics[width=0.24\textwidth]{Figures/bar_Z_15000.eps}
    \includegraphics[width=0.24\textwidth]{Figures/bar_Z_20000.eps}
    \caption{}
    \label{fig:RZ}
    \end{subfigure}

    \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=0.24\textwidth]{Figures/bar_T_05000.eps}
    \includegraphics[width=0.24\textwidth]{Figures/bar_T_10000.eps}
    \includegraphics[width=0.24\textwidth]{Figures/bar_T_15000.eps}
    \includegraphics[width=0.24\textwidth]{Figures/bar_T_20000.eps}
    \caption{}
    \label{fig:RT}
    \end{subfigure}

    \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=0.24\textwidth]{Figures/bar_CO_05000.eps}
    \includegraphics[width=0.24\textwidth]{Figures/bar_CO_10000.eps}
    \includegraphics[width=0.24\textwidth]{Figures/bar_CO_15000.eps}
    \includegraphics[width=0.24\textwidth]{Figures/bar_CO_20000.eps}
    \caption{}
    \label{fig:RCO}
    \end{subfigure}

    \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=0.24\textwidth]{Figures/bar_CO2_05000.eps}
    \includegraphics[width=0.24\textwidth]{Figures/bar_CO2_10000.eps}
    \includegraphics[width=0.24\textwidth]{Figures/bar_CO2_15000.eps}
    \includegraphics[width=0.24\textwidth]{Figures/bar_CO2_20000.eps}
    \caption{}
    \label{fig:RCO2}
    \end{subfigure}

    \caption{Reynolds-averaged mean and RMS values of the mixture fraction ($Z$), temperature ($T$), CO mass fraction ($Y_{CO}$), and CO\textsubscript{2} mass fraction ($Y_{CO_2}$). Lines and symbols denote LES and  DNS results, respectively.}
    \label{fig:RZTC}
\end{figure}
  

\begin{figure}
    \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.3\textwidth]{Figures/SliceXZ_CO_DNS_0000.png}
         \includegraphics[width=0.3\textwidth]{Figures/SliceXZ_CO_LES_0000.png}
         \caption{$t=20tj$}
         %\caption{}
         \label{fig:COSlicesXZ20}
     \end{subfigure}
     
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.3\textwidth]{Figures/SliceXZ_CO_DNS_0001.png}
         \includegraphics[width=0.3\textwidth]{Figures/SliceXZ_CO_LES_0001.png}
         \caption{$t=40tj$}
         %\caption{}
         \label{fig:COSlicesXZ40}
     \end{subfigure}
    
    \caption{Instantaneous slice plots at $y=0$ of CO mass fraction obtained from DNS (left) and LES-FDF (right).}
    \label{fig:COSlicesXZ}
\end{figure}

